Scalable Gradients for Stochastic Differential Equations

The adjoint sensitivity method scalably computes gradients of solutions to ordinary differential equations. We generalize this method to stochastic differential equations, allowing time-efficient and constant-memory computation of gradients with high-order adaptive solvers. Specifically, we derive a stochastic differential equation whose solution is the gradient, a memory-efficient algorithm for caching noise, and conditions under which numerical solutions converge. In addition, we combine our method with gradient-based stochastic variational inference for latent stochastic differential equations. We use our method to fit stochastic dynamics defined by neural networks, achieving competitive performance on a 50-dimensional motion capture dataset.

==> abstract_aabi.tex <==
\begin{abstract}
We derive reverse-mode automatic differentiation for solutions of stochastic differential equations (SDEs), allowing time-efficient and constant-memory computation of pathwise gradients.
Specifically, we construct a backward SDE whose solution is the gradient and provide conditions under which numerical solutions converge.
We combine our stochastic adjoint approach with a stochastic variational inference scheme for continuous-time latent SDE models and learn distributions over functions using stochastic gradient descent.
Our latent SDE model achieves competitive performance compared to existing approaches on time series modeling.
\end{abstract}


==> bnn.tex <==
\section{Infinitely Deep Bayesian Neural Networks}

The limit of a residual network as the size of each layer's update goes to zero is an ODE:
\begin{align}
z_{t+1} = z_t + h f(z_t, \theta(t)) \quad \implies \quad \frac{\partial z(t)}{(\partial t)} = f(z_t, \theta(t))
\end{align}
Analogously, the limit of a Bayesian neural network, in which there is uncertainty about the weights of each layer, is an SDE.
Specifically, if the prior on each layer's weights is independent with mean $\mu$ and variance $\sigma^2$, then in the infinitesimal limit, $\theta(\cdot)$ becomes a white noise process.
By Ito's lemma,
\begin{align}
d z = f(z_t, \theta(t))
\end{align}

